Jack of All Tasks, Master of Many: Designing General-purpose Coarse-to-Fine Vision-Language Model

The ability of large language models (LLMs) to process visual inputs has given rise to general-purpose vision systems, unifying various vision-language (VL) tasks by instruction tuning. However, due to the enormous diversity in input-output formats in the vision domain, existing general-purpose models fail to successfully integrate segmentation and multi-image inputs with coarse-level tasks into a single framework. In this work, we introduce VistaLLM, a powerful visual system that addresses coarse- and fine-grained VL tasks over single and multiple input images using a unified framework. VistaLLM utilizes an instruction-guided image tokenizer that filters global embeddings using task descriptions to extract compressed and refined features from numerous images. Moreover, VistaLLM employs a gradient-aware adaptive sampling technique to represent binary segmentation masks as sequences, significantly improving over previously used uniform sampling. To bolster the desired capability of VistaLLM, we curate CoinIt, a comprehensive coarse-to-fine instruction tuning dataset with 6.8M samples. We also address the lack of multi-image grounding datasets by introducing a novel task, AttCoSeg (Attribute-level Co-Segmentation), which boosts the model's reasoning and grounding capability over multiple input images. Extensive experiments on a wide range of V- and VL tasks demonstrate the effectiveness of VistaLLM by achieving consistent state-of-the-art performance over strong baselines across all downstream tasks. Our project page can be found at https://shramanpramanick.github.io/VistaLLM/.

==> extra_tables.tex <==

\begin{table*}[!t]
\centering

\small
\setlength{\tabcolsep}{2pt}
\resizebox{\textwidth}{!}{\begin{tabular}{@{}l c c c c | c c c | c c c c c c @{}}

\toprule
\multirow{3}{*}{\textbf{Model}} & \multicolumn{4}{c|}{\multirow{1}{*}{\textbf{Input Type}}} & \multicolumn{3}{c|}{\multirow{1}{*}{\textbf{Image-level Tasks}}} & \multicolumn{6}{c}{\multirow{1}{*}{\textbf{Region-level Tasks}}}  \\ 
\cmidrule{2-5} \cmidrule{6-8} \cmidrule{9-14}
& \multirow{2}{1.1cm}{\centering Multiple Images} & \multicolumn{3}{c|}{\centering Large Number of} & \multirow{2}{1.0cm}{VQA \& Caption} & \multicolumn{2}{c|}{\centering Reasoning} & \multirow{2}{1.0cm}{\centering Dense QA} & \multicolumn{2}{c}{\centering Single-obj.} & \multicolumn{2}{c}{\centering Multi-obj.} & \multirow{2}{1.375cm}{\centering Multi Img. Co-Seg.} \\

& & \centering Points & \centering Boxes & Masks & & One Img. & Multi Img. & & \centering Det. & Seg. & Det. & Seg. &  \\
\midrule

LLaVa \cite{liu2023llava} \\
InstructBLIP \\
GPT4RoI \\
Vision-LLM \\
Shikra \\
Ferret \\
MiniGPT-v2 \\
\rowcolor{Light}
Ours & & & & & & & & & & & & & \\

\bottomrule
\end{tabular}}
\caption{}\label{tab:comparison_baselines}
\vspace{-2mm}
\end{table*}

\begin{table*}[!t]
\centering

\small
\setlength{\tabcolsep}{4pt}
\resizebox{\textwidth}{!}{\begin{tabular}{l c | c c c c c c c c | l c | c c c c c c c c}

\toprule 

\multicolumn{10}{c|}{\bf Referring Expression Comprehension (REC)} & \multicolumn{10}{c}{\bf Referring Expression Segmentation (RES)} \\

\multirow{2}{*}{\bf Method} & \multirow{2}{1.1 cm}{\bf \centering Unified?} & \multicolumn{3}{c}{Ref} & \multicolumn{3}{c}{Ref+} & \multicolumn{2}{c|}{Refg} & \multirow{2}{*}{\bf Method} & \multirow{2}{*}{\bf \centering Unified?} & \multicolumn{3}{c}{Ref} & \multicolumn{3}{c}{Ref+} & \multicolumn{2}{c}{Refg}  \\ 

& & val & testA & testB & val & testA & testB & \centering val & \centering test & & & val & testA & testB & val & testA & testB & val & test  \\

\midrule 

% TransVG \cite{} & \ding{55} & 81.02 & 82.72 & 78.35 & 64.82 & 70.70 & 56.94 & 68.67 & 67.73\\ 
VILLA \cite{gan2020large} & \ding{55} & 82.4 & 87.5 & 74.8 & 76.2 & 81.5 & 66.8 & 76.2 & 76.7 & CRIS \cite{wang2022cris} & \ding{55} & 70.5 & 73.2 & 66.1 & 62.3 & 68.1 & 53.7 & 59.9 & 60.4 \\
UniTAB \cite{yang2022unitab} & \ding{55} & 86.3 & 88.8 & 80.6 & 78.7 & 83.2 & 69.5 & 80.0 & 80.0 & SeqTR \cite{zhu2022seqtr} & \ding{55} & 71.7 & 73.3 & 69.8 & 63.0 & 66.7 & 59.0 & 64.7 & 65.7 \\
MDETR \cite{kamath2021mdetr} & \ding{55} & 86.8 & 89.6 & 81.4 & 79.5 & 84.1 & 70.6 & 81.6 & 80.9 & VLT \cite{liu2022instance} & \ding{55} & 73.0 & 76.0 & 69.6 & 63.5 & 68.4 & 56.9 & 63.5 & 66.2 \\ 
PolyFormer-B \cite{liu2023polyformer} & \ding{55} & 89.7 & 91.7 & 86.0 & 83.7 & 88.6 & 76.4 & 84.5 & 85.0 & RefTr \cite{li2021referring} & \ding{55} & 74.3 & 76.8 & 70.9 & 66.8 & 70.6 & 59.4 & 66.6 & 67.4 \\
OFA-L \cite{wang2022ofa} & \ding{51} & 80.0 & 83.7 & 76.4 & 68.3 & 76.0 & 61.8 & 67.6 & 67.6 & LAVT \cite{yang2022lavt} & \ding{55} & 74.5 & 76.9 & 70.9 & 65.8 & 71.0 & 59.2 & 63.3 & 63.6 \\
VisionLLM-H \cite{wang2023visionllm} & \ding{51} & $-$ & 86.7 & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & PolyFormer-B \cite{liu2023polyformer} & \ding{55} & 76.0 & 77.1 & 73.2 & 70.7 & 74.5 & 64.6 & 69.4 & 69.9 \\
Shikra7B \cite{chen2023shikra} & \ding{51} & 87.0 & 90.6 & 80.2 & 81.6 & 87.4 & 72.1 & 82.3 & 82.2 & GRES \cite{liu2023gres} & \ding{55} & 73.8 & 76.5 & 70.2 & 66.0 & 71.0 & 57.7 & 65.0 & 66.0 \\
MiniGPT-v2 \cite{chen2023minigptv2} & \ding{51} & 88.7 & 91.7 & 85.3 & 80.0 & 85.1 & 74.5 & 84.4 & 84.7 & LISA7B \cite{lai2023lisa} & \ding{55} & 74.9 & 79.1 & 72.3 & 65.1 & 70.8 & 58.1 & 67.9 & 70.6 \\
\rowcolor{Light}
\model & & & \\





\bottomrule
\end{tabular}}
\caption{} \label{}
\vspace{-2mm}
\end{table*}




\begin{table}[!t]
\centering

\small
\setlength{\tabcolsep}{4pt}
\resizebox{0.9\columnwidth}{!}{\begin{tabular}{l | c c c c c c c c c}

\toprule 


\multirow{2}{0.5cm}{\bf Method} & \multicolumn{3}{c}{Random} & \multicolumn{3}{c}{Popular} & \multicolumn{3}{c}{Adversarial}  \\ 

& Prec. & Recall & F1 & Prec. & Recall & F1 & Prec. & Recall & F1 \\

\midrule

mPLUG-Owl & 52.1 & 99.6 & 68.4 & 50.5 & 99.4 & 66.9 & 50.3 & \bf 99.3 & 66.8 \\
% MM-GPT & 50.5 & 100.0 & 66.7 & 50.0 & 100.0 & 66.7 & 50.0 & 100.0 & 66.7 \\
LLaVA \cite{liu2023llava} & 50.2 & 99.1 & 66.6 & 49.9 & 99.3 & 66.4 & 49.9 & 99.1 & 66.3 \\
MiniGPT4 \cite{zhu2023minigpt} & 78.2 & 82.2 & 80.2 & 65.9 & 81.9 & 73.0 & 61.2 & 82.9 & 70.4 \\
InstructBLIP \cite{instructblip} & 84.1 & 95.1 & 89.3 & 76.3 & 95.1 & \bf 84.7 & 65.1 & 95.1 & 77.3 \\
Shikra \cite{chen2023shikra} & 94.4 & 79.3 & 86.2 & 87.6 & 79.2 & 83.2 & 85.6 & 79.6 & 82.5 \\


\rowcolor{Light}
\model-13B & \bf 96.1 & \bf 82.0 & \bf 88.5 & \bf 88.0 & \bf 80.8 & 84.2 & \bf 85.9 & 80.2 & \bf 83.0 \\
\bf \textcolor{blue}{$\Delta_{\text{Ours - Shikra}}$} & \textcolor{blue}{1.7} \textcolor{blue}{$\uparrow$} & \textcolor{blue}{2.7} \textcolor{blue}{$\uparrow$} & \textcolor{blue}{2.3} \textcolor{blue}{$\uparrow$} & \textcolor{blue}{0.4} \textcolor{blue}{$\uparrow$} & \textcolor{blue}{1.6} \textcolor{blue}{$\uparrow$} & \textcolor{blue}{1.0} \textcolor{blue}{$\uparrow$} & \textcolor{blue}{0.3} \textcolor{blue}{$\uparrow$} & \textcolor{blue}{0.6} \textcolor{blue}{$\uparrow$} & \textcolor{blue}{0.5} \textcolor{blue}{$\uparrow$} \\

\bottomrule
\end{tabular}}
\caption{POPE} \label{tab:pope}
\vspace{-2mm}
\end{table}



\begin{table}[!t]
\centering

\small
\setlength{\tabcolsep}{4pt}
\resizebox{0.45\columnwidth}{!}{\begin{tabular}{l c | c c}

\toprule 


\multirow{2}{0.5cm}{\bf Method} & \multirow{2}{1.21cm}{\bf \centering General-purpose?} & \multicolumn{2}{c}{\bf NLVR}  \\ 

& & dev & test-P \\

\midrule

VisualBERT \cite{li2019visualbert} & \ding{55} & 67.4 & 67.0 \\
LXMERT \cite{tan2019lxmert} & \ding{55} & 74.9 & 74.5 \\
SOHO \cite{huang2021seeing} & \ding{55} & 76.3 & 77.3\\
Oscar \cite{li2020oscar} & \ding{55} & 78.1 & 78.4 \\
Uniter \cite{chen2020uniter} & \ding{55} & 77.2 & 77.9 \\
VILLA \cite{gan2020large} & \ding{55} & 78.4 & 79.3 \\
ALBEF \cite{li2021align} & \ding{55} & \underline{80.2} & \underline{80.5} \\
% METER \cite{dou2022empirical} & \ding{55} & \bf 82.2 & \bf 83.5 \\
% FIBER \cite{dou2022coarse} & \ding{55} & \bf 84.6 & \bf 85.5 \\
\rowcolor{Light}
\model & \ding{51} & \bf{80.7} & \bf{81.1} \\

\midrule

% \bf \textcolor{blue}{$\Delta_{\text{Ours - METER}}$} & $-$ & \textcolor{Brown}{1.5} \textcolor{Brown}{$\downarrow$} & \textcolor{Brown}{2.4} \textcolor{Brown}{$\downarrow$} \\
\bf \textcolor{blue}{$\Delta_{\text{Ours - ALBEF}}$} & $-$ & \textcolor{blue}{0.5} \textcolor{blue}{$\uparrow$} & \textcolor{blue}{0.6} \textcolor{blue}{$\uparrow$} \\

\bottomrule
\end{tabular}}
\caption{\textbf{Results on NLVR.} \model\ is the first general-purpose model to address NLVR, and beats strong fine-tuned models.} \label{tab:nlvr}
\vspace{-2mm}
\end{table}


\begin{table}[!t]
\centering

\small
\setlength{\tabcolsep}{4pt}
\resizebox{0.65\columnwidth}{!}{\begin{tabular}{l | c c c c c c}

\toprule 


\multirow{2}{0.5cm}{\bf Method} & \multicolumn{2}{c}{Random} & \multicolumn{2}{c}{Popular} & \multicolumn{2}{c}{Adv.}  \\ 

& Acc. & F1 & Acc. & F1 & Acc. & F1 \\

\midrule

mPLUG-Owl & 54.0 & 68.4 & 50.9 & 66.9 & 50.7 & 66.8 \\
% MM-GPT & 50.5 & 100.0 & 66.7 & 50.0 & 100.0 & 66.7 & 50.0 & 100.0 & 66.7 \\
LLaVA \cite{liu2023llava} & 50.4 & 66.6 & 49.9 & 66.4 & 49.7 & 66.3 \\
MiniGPT4 \cite{zhu2023minigpt} & 79.7 & 80.2 & 69.7 & 73.0 & 65.2 & 70.4 \\
InstructBLIP \cite{instructblip} & 88.6 & 89.3 & 82.8 & 84.7 & 72.1 & 77.3 \\
Shikra-7B \cite{chen2023shikra} & 86.9 & 86.2 & 84.0 & 83.2 & \underline{83.1} & 82.5 \\
Ferret-13B \cite{you2023ferret} & \bf 90.2 & \underline{89.8} & \underline{84.9} & 84.2 & 82.4 & 82.0 \\


\rowcolor{Light}
\model-13B & \underline{89.8} & \bf 90.5 & \bf 85.3 & \bf 84.8 & \bf 83.5 & \bf 82.9 \\
\midrule
\bf \textcolor{blue}{$\Delta_{\text{Ours - Ferret-13B}}$} & \textcolor{Brown}{0.4} \textcolor{Brown}{$\downarrow$} & \textcolor{blue}{0.7} \textcolor{blue}{$\uparrow$} & \textcolor{blue}{0.4} \textcolor{blue}{$\uparrow$} & \textcolor{blue}{0.6} \textcolor{blue}{$\uparrow$} & \textcolor{blue}{1.1} \textcolor{blue}{$\uparrow$} & \textcolor{blue}{0.9} \textcolor{blue}{$\uparrow$} \\

\bottomrule
\end{tabular}}
\caption{\textbf{Performance on object hallucination benchmark using POPE evaluation pipeline} \cite{li2023evaluating}. \model\ demonstrates an intriguing property of alleviating object hallucinations.} \label{tab:pope}
\vspace{-2mm}
\end{table}





%%% Supplementary


\begin{table*}[!t]
\centering

\small
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.08}
\resizebox{\textwidth}{!}{\begin{tabular}{@{} c l | c c c c | c c c | c c c c c c c @{}}

\toprule
& \multirow{3}{*}{\textbf{Model}} & \multicolumn{4}{c|}{\multirow{1}{*}{\textbf{Input Type}}} & \multicolumn{3}{c|}{\multirow{1}{*}{\textbf{Image-level Tasks}}} & \multicolumn{7}{c}{\multirow{1}{*}{\textbf{Region-level Tasks}}}  \\ 
\cmidrule{3-16}
& & \multirow{2}{1.15cm}{\centering Multiple Images} & \multirow{2}{*}{Points} & \multirow{2}{*}{Boxes} & \multirow{2}{*}{Masks} & \multirow{2}{1.5cm}{VQAv2 \& Captioning} & \multicolumn{2}{c|}{\centering Reasoning over} & \multirow{2}{*}{BoxQA} & \multirow{2}{*}{PointQA} & \multicolumn{2}{c}{\centering Single Instance} & \multicolumn{2}{c}{\centering Multi Instance} & \multirow{2}{*}{\centering CoSeg} \\

& & & & & & & Single Image & Multi Image & & & \centering Detection & Segmentation & \centering Detection & Segmentation &  \\
\midrule

\multirow{4}{1.2cm}{\centering Two-Stage} & Visual ChatGPT \cite{wu2023visual} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{51} & \ding{51} & \ding{55} & \ding{55} & \ding{55} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{55}  \\

& BuboGPT \cite{zhao2023bubogpt}  & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{51} & \ding{51} & \ding{55} & \ding{55} & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{55} \\

& DetGPT \cite{pi2023detgpt} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{51} & \ding{51} & \ding{55} & \ding{55} & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{55}\\


& LISA \cite{lai2023lisa} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{51} & \ding{51} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{51} & \ding{55} & \ding{55} & \ding{55} \\


\midrule

\multirow{12}{1.2cm}{\centering End-to-End} & LLaVa \cite{liu2023llava} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{51} & \ding{51} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} \\


& InstructBLIP \cite{instructblip} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{51} & \ding{51} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} \\


& GPT4RoI \cite{zhang2023gpt4roi} & \ding{55} & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} \\


& KOSMOS-2 \cite{peng2023kosmos2} & \ding{55} & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{55} \\

& VisionLLM \cite{wang2023visionllm} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{51} & \ding{51} & \ding{55} & \ding{55} & \ding{55} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{55} \\

& Shikra \cite{chen2023shikra} & \ding{55} & \ding{51} & \ding{51} & \ding{55} & \ding{51} & \ding{51} & \ding{55} & \ding{51} & \ding{51} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{55}  \\

& PVIT \cite{chen2023position} & \ding{55} & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} & \ding{55} \\

& CogVLM \cite{wang2023cogvlm} & \ding{55} & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{55} \\

& COMM \cite{jiang2023comm} & \ding{55} & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{55} \\

& MiniGPT-v2 \cite{chen2023minigptv2} & \ding{55} & \ding{51} & \ding{51} & \ding{55} & \ding{51} & \ding{51} & \ding{55} & \ding{51} & \ding{51} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{55} \\

& Ferret \cite{you2023ferret} & \ding{55} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{51} & \ding{55} & \ding{51} & \ding{51} & \ding{51} & \ding{55} & \ding{51} & \ding{55} & \ding{55} \\


& \CC{}\model\ & \CC{}\ding{51} & \CC{}\ding{51} & \CC{}\ding{51} & \CC{}\ding{51} & \CC{}\ding{51} & \CC{}\ding{51} & \CC{}\ding{51} & \CC{}\ding{51} & \CC{}\ding{51} & \CC{}\ding{51} & \CC{}\ding{51} & \CC{}\ding{51} & \CC{}\ding{51} & \CC{}\ding{51} \\

\bottomrule
\end{tabular}}
\caption{\textbf{Comparison of \model\ vs existing general-purpose vision systems.} \model\ integrates a wide range of image-level and region-level vision-language reasoning and grounding tasks over single and multiple input images into a unified framework.}
\label{tab:comparison_baselines}
\vspace{-2mm}
\end{table*}

==> graphs/plot_1.tex <==
\begin{figure}[!t]
    \centering
    \hspace{-0em}
    \begin{subfigure}[b]{0.495\linewidth}
        \resizebox{1.0\textwidth}{!}{
            \input{graphs/mIoU_upper_bound}%
        }
        \caption{\textbf{mIoU upper bound} on RES Ref val with number of sampled points.}
        \label{fig:sampling_ablation_1}
    \end{subfigure}
 \hspace{-0em}
    \begin{subfigure}[b]{0.495\linewidth}
        \resizebox{1.0\textwidth}{!}{
            \input{graphs/mIoU}%
        }
        \caption{\textbf{mIoU by \model} on RES with number of sampled points.}
        \label{fig:sampling_ablation_2}
    \end{subfigure}
\vspace{-2mm}
\caption{\textbf{Ablative experiments on RES task.} (a) Comparison of the highest possible mIoU by adaptive and uniform sampling, proving the lesser information loss in adaptive sampling. (b) Effect of number of sampled points on the performance of \model.}
\label{fig:sampling_ablation}
\vspace{-5mm}
\end{figure}

==> preamble.tex <==
%
% --- inline annotations
%

% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}


